TPRF: A Transformer-based Pseudo-Relevance Feedback Model for Efficient and Effective Retrieval

This paper considers Pseudo-Relevance Feedback (PRF) methods for dense retrievers in a resource constrained environment such as that of cheap cloud instances or embedded systems (e.g., smartphones and smartwatches), where memory and CPU are limited and GPUs are not present. For this, we propose a transformer-based PRF method (TPRF), which has a much smaller memory footprint and faster inference time compared to other deep language models that employ PRF mechanisms, with a marginal effectiveness loss. TPRF learns how to effectively combine the relevance feedback signals from dense passage representations. Specifically, TPRF provides a mechanism for modelling relationships and weights between the query and the relevance feedback signals. The method is agnostic to the specific dense representation used and thus can be generally applied to any dense retriever.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> relatedwork.tex <==
\section{Related Works}

%Pseudo-Relevance Feedback (PRF) is a classic query expansion technique that aims to mitigate the mismatch between query intent and query representation~\cite{clinchant2013a,wang2020pseudo}. A classic PRF framework often utilises the top-ranked passages from the initial retrieved results and assumes these passages are relevant or at least contains the relevant information, then these passages are used to select additional terms to be added to the original query or adjusting the original query vector weights to obtain the new query representation. Many classic PRF models such as Rocchio~\cite{rocchio1971rocchio}, query-regularized mixture model~\cite{tao2006regularized}, RM3~\cite{lv2009comparative}, relevance-feedback matrix factorization~\cite{zamani2016pseudo}, and relevance models~\cite{lavrenko2017relevance} have been well studied on top of traditional bag-of-words retrieval models. These traditional PRF methods are simple but more robust and generalisable in comparison to more complex models~\cite{tao2006regularized,zamani2016pseudo}, which have only achieved marginal gains and difficult to implement/reproduce on other datasets or domains than those in which they have been originally evaluated. From previous research, the classic PRF methods have shown to be effective for improving retrieval effectiveness~\cite{clinchant2013a,lavrenko2017relevance} thus common in information retrieval systems. 

Next we review some representative neural methods for PRF, with a particular attention to those for dense retrievers.

\vspace{4pt}
\textbf{Neural PRF Methods.}
\citet{li2018nprf}'s neural PRF framework, further extended by~\citet{wang2020end}, adopts a feed-forward neural network to aggregate the target query and the target feedback relevance scores to obtain the relevance score of the target document. These methods however achieve only marginal improvements over bag-of-words methods. %(BM25).

\citet{padaki2020rethinking} combined RM3 with monoBERT~\cite{nogueira2019passage}: RM3 is used to select feedback terms that are appended to the textual input that is provided to the monoBERT ranker. This however has not led to a more effective ranking; it also presents the same computational challenges presented by monoBERT.

%Other than the well-studied classic PRF approaches, recently, researchers have been studying different PRF approaches. \citet{lin2019simplest} treated the document ranking task as a binary classification task. In this approach, the authors introduced positive and negative pseudo labels, where the top-$k$ documents from the initial retrieved results are treated as positive labels, the bottom-$n$ documents from the initial retrieved results are treated as negative labels. A linear interpolation of the classifier and initial retrieval scores is used to obtain the final score of a document. Another approach proposed by~\citet{li2018nprf} is a neural PRF framework, which was further extended by~\cite{wang2020end}. For this approach, the authors adopted a feed-forward neural network to aggregate the target query and the target feedback relevance scores to obtain the relevance score of the target document. According to their results, the proposed approach achieved marginal improvements compared to the BM25 baseline. On the other hand, the efficiency of the proposed model is not reported, therefore, these marginal improvements might be at the cost of efficiency.

%Recently, deep language models based on transformers~\cite{vaswani2017attention} have achieved significant improvements or even become the state-of-the-art over a series of tasks, including information retrieval. Different deep language models, such as BERT~\cite{devlin2018bert}, RoBERTa~\cite{liu2019roberta}, and T5~\cite{raffel2019exploring}, have been adopted to the document ranking tasks and have shown promising improvements. BERT, in specific, is the first deep language model that is adapted to the ranking task, and have shown improvements over the previous state-of-the-art model~\cite{nogueira2019passage}. Because of the fact that PRF approaches can also improve the search effectiveness, recent research also considered integrating PRF mechanism with deep language models. 

\citet{yu2021pgt} represents a feedback passage as a node in a Graph-based Transformer (PGT) and the PRF signals are obtained using the sparse attention mechanism between the nodes in the graph. 
While the improvements gained from this approach are marginal, its memory and computational costs are high.
An advantage of this method, compared for example to ANCE-PRF~\cite{yu2021improving,li2021improving} is that the PRF mechanism is not constrained by the input-size limit of the underlying deep language model used in the PRF encoder. Our method, TPRF, also is not limited in PRF input size.

%\citet{yu2021pgt} proposed a PRF framework that utilises the PRF and a Graph-based Transformer (PGT). In this approach, each feedback passage is represented by a node in the graph, the PRF signals are obtained by using sparse attention between the graph nodes. With this framework, the PRF mechanism does not constrained by the input-size limit of the deep language models. However, the improvements gained from this approach is marginal compared to the baselines, but at a huge cost of efficiency and computation. \citet{padaki2020rethinking} tried to integrate RM3 with BERT model. Based on the results, by expanding the query via RM3 and add additional terms to the original query significantly hurts the effectiveness of a fine-tuned BERT reranker.

\citet{zheng-etal-2020-bert,zheng2021contextualized} proposed a three-phase PRF method, called BERT-QE. The first phase corresponds to the monoBERT ranker~\cite{nogueira2019passage}, which is used to produce a first ranking of which the top-$k$ passages are used for the second phase. In the  second phase, the text of top-$k$ passages are split into overlapping partitions using a sliding window. Then, the text of each partition is concatenated to that of the original query and given as input to monoBERT to produce a re-ranking of the partition. From the re-ranked partitions, the text of the top-$m$ passages are selected in the third phase and provided as input to monoBERT to produce a final ranking:  the final score of a candidate passage is the linear interpolation of the monoBERT score from first phase and the third phase. While BERT-QE achieves significant effectiveness improvements over monoBERT, it also requires more than 11.01x more computations, rendering this method largely infeasible in many search settings, let along in the resource-constrained setting we consider in this paper.





%More recently, \citet{zheng-etal-2020-bert,zheng2021contextualized} proposed a BERT-QE model based on BERT that consists of three phases. The first phase is a standard BM25+BERT reranking that is the same as the model proposed in~\cite{nogueira2019passage}. For the second phase, top-$k$ passages are treated as relevant passages and splitted into overlapping partitions with sliding window technique. Then each of the partition are passed to BERT reranker again along with the original query to rerank the partitions. From the reranked partitions, top-$m$ are selected and pass to BERT again with the candidate passage for a third round of reranking. The score of a candidate passage is calculated as a weighted sum where the weight is the relevance score from the second phase. The final score of a candidate passage is a linear interpolation of the BERT score from first phase and the third phase weighted sum score. According to the results from the authors, BERT-QE achieved significant improvements over BERT reranker w.r.t the effectiveness, it also requires more than 11.01x more computations compared to BERT, which is infeasible to be applied in many practical settings.

\citet{wang2020pseudo} proposed a PRF framework that considers both relevance matching signals, derived from a bag-of-words model like BM25, and semantic matching signals. For computing the semantic matching signal, the text of the top-$k$ passages is split into sentences, and for each sentence, monoBERT is used to compute the relevance  between the sentence and the query. The top-$m$ scores from a single passage are treated as the semantic scores for this passage. 
A linear interpolation of the semantic score and the relevance score is then used to obtain a final score for each passage. Then, expansion terms from the top ranked passages are extracted and added to the original query, and a new round of retrieval is performed. This method results in marginal improvements in search effectiveness, but at the expenses of large computational costs.



%Another different approach from \citet{wang2020pseudo} argues that the current PRF frameworks only consider the relevance matching, which is mainly based on the term matching mechanism. One big challenge of relevance matching approach is that it cannot capture the semantic meaning of the term, especially when a same term has different meanings. Therefore, the authors proposed a PRF framework that considers both relevance matching and semantic matching. For the relevance matching, the authors are using classic BM25 retrieval model. For semantic matching, they split the top-$k$ passages into sentences, for each sentence, they use BERT model to estimate the semantic relevance score between the sentence and the query. Top-$m$ scores from a same passage are treated as the semantic score of this passage. A linear interpolation of the semantic score and the relevance score is used to obtain the final score for each passage. Based on this score, the authors extracted the expansion terms from the top reranked passages and added to the original query, then a subsequent retrieval is performed to get the final ranked results. The proposed framework have shown that deep language models can identify relevance signals from the feedback passages, although the improvement is marginal compare to the baselines. On the other hand, the proposed framework uses BERT reranker at sentence level, which adds a huge amount of inference time, the marginal improvements are at a large cost of efficiency.

\vspace{4pt}
\textbf{Dense Retrievers PRF Methods.}
Most of the previous PRF methods are characterised by prohibitive computational requirements and query latencies. Dense retrievers based PRF methods attempt to overcome these limitations.  

\citet{li2021pseudo} proposed a the Vector-based PRF framework for dense retrievers: this is instantiated into two simple but effective PRF approaches (Rocchio-PRF and Average-PRF) that are agnostic to the specific dense retriever used. Both methods use the dense vectors associated to the feedback passages and combine this with the dense vector of the encoded query to generate a new query representation for re-ranking.
Average-PRF does this through a simple average of the input dense vectors, while Rocchio-PRF does a parametrised weighted sum of the dense query vector and the dense feedback passage vectors.
These vector-based operations are highly efficient and no new BERT encoding inference is required, making these methods highly effective, whilst also proving able to achieve significant improvements over baseline dense retrievers. However, to achieve the highest effectiveness gain, tuning of the Rocchio-PRF parameters is required, which may be challenging is contexts with limited data or scarce computational resources for tuning.


%Because previous deep language models, such as BERT, is very expensive at inference time, dense retrievers becomes more popular cause its significant efficiency improvements compares to previous deep language models~\cite{xiong2020approximate,zhan2020repbert,lin2020distilling}. \citet{li2021pseudo} proposed a PRF framework based on the dense retrievers which uses two simple PRF approaches based on different dense retrievers, including two state-of-the-art models, namely Rocchio-PRF and Average-PRF. For Rocchio-PRF, the authors are inspired by the traditional Rocchio PRF method~\cite{rocchio1971rocchio}. To obtain the new query representation, the authors use a weighted sum of the query vector and top-$k$ passage vectors from the initial retrieval, in the aim to move the query vector to the top-$k$ feedback passage vectors. For Average-PRF, the authors simply take an average of the query vector and the feedback passage vectors to obtain the new query representation. For both approaches, after obtaining the new query representation, a subsequent retrieval is performed to get the final results. Compared to previous complex frameworks, the model proposed is much efficient and achieved significant improvements over several evaluation metrics across different datasets and solves the input limitation of the deep language models. However, to achieve the highest effectiveness gain, one needs to tune the Rocchio parameters to adjust the weights of query vector and feedback passage vectors, which is time-consuming.

\citet{yu2021improving} devised a PRF method based on dense retriever ANCE~\cite{xiong2020approximate}, ANCE-PRF, which has been later expanded to any dense retriever by ~\citet{li2021improving}. The method trains a new ANCE query encoder on the top-$k$ feedback passages. These passages are taken from the initial ANCE run and their text is concatenated to that of the original query. This combined text is then encoded into a new dense representation using the ANCE-PRF encoder (a finetuned ANCE query encoder for the PRF task), while the ANCE passage encoder is left unchanged. The representation produced by the ANCE-PRF encoder is used for ranking passages. Empirical evaluation have demonstrated this method delivers significant search effectiveness improvements. However it is limited in the size of the PRF signal it can handle~\cite{li2021improving}: the ANCE-PRF model inherits the input limitation constraints of the underlying RoBERTa deep language model. On TREC DL and MS MARCO this means that up to a maximum of about 7 passages can be considered as PRF signal: after that, any additional feedback passage is ignored. The TPRF method we propose in this paper circumvents this limitation, as it works in the dense representations space and not in the input texts space. Another limitation of ANCE-PRF is that the underlying training does not generalise well across other dense retrievers~\cite{li2021improving}: the training parameters need to be adjusted accordingly for different dense retrievers, and improvements can vary largely among dense retrievers. 



%
%In this framework, a new ANCE query encoder based on the original one. The new query encoder takes top-$k$ feedback passages from the initial ANCE retrieval and concatenate the original query text with the feedback passage texts to form the new query representation, meanwhile, the passage encoder remains the same. Then this new query text is passed to the trained ANCE-PRF encoder to obtain the new query representation, this new representation is used to perform a subsequent retrieval and get the final results. The results reported by the authors shown that the improvements are significant over several evaluation metrics across different datasets, however, according to a recent reproducibility paper from~\citet{li2021improving}, the ANCE-PRF model inherits the input limitation constraint from the deep language models, because of the concatenation of query text and feedback passage texts, the PRF depth is maxed at 7 on the datasets the authors used. Another limitation is that ANCE-PRF does not generalise well on other dense retrievers, the training parameters need to be adjusted accordingly w.r.t different dense retrievers, which makes it very difficult to have the same effectiveness improvements as shown with ANCE-PRF.
%



==> results-old.tex <==
\section{Results}\label{sec:results}
%In this section, we investigate how TPRF compares to other dense retriever PRF models in terms of model size (RQ1), query latency (RQ2), and effectiveness (RQ3).

%address the following research questions:
%\begin{itemize}
%\item[RQ1] How does TPRF compare to other dense retriever PRF models in terms of the model size
%\item[RQ2] How does TPRF compare to other dense retriever PRF models in terms of efficiency
%\item[RQ3] How does TPRF compare to other dense retriever PRF models in terms of effectiveness
%\end{itemize}

% RQ2: ... in terms of inference time (efficiency) (How K affects efficiency)

\subsection{Comparison w.r.t. Model Size}


%\begin{figure}
%	\centering
%	\begin{subfigure}[b]{0.22\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{figures/TPRF-Latency-Space-Effectiveness -ANCE-2019-n.pdf}
%		\caption{$y=x$}
%		\label{fig:y equals x}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.22\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{figures/TPRF-Latency-Space-Effectiveness -ANCE-2019-r.pdf}
%		\caption{$y=3sinx$}
%		\label{fig:three sin x}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.22\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{figures/TPRF-Latency-Space-Effectiveness -ANCE-2020-n.pdf}
%		\caption{$y=5/x$}
%		\label{fig:five over x}
%	\end{subfigure}
%\hfill
%	\begin{subfigure}[b]{0.22\textwidth}
%	\centering
%	\includegraphics[width=\textwidth]{figures/TPRF-Latency-Space-Effectiveness -ANCE-2020-r.pdf}
%	\caption{$y=5/x$}
%	\label{fig:five over x}
%\end{subfigure}
%	\caption{Three simple graphs}
%	\label{fig:three graphs}
%\end{figure}
%
%
%




%\begin{figure}
%	\centering
%	\begin{subfigure}{\columnwidth}
%	\includegraphics[width=\columnwidth]{figures/TPRF-Spaces-ANCE-Effectiveness_trec_dl_2019.pdf}
% 	\caption{TREC DL 2019}
%	\label{fig:spaces-trec-2019}
%	\end{subfigure}
%	\begin{subfigure}{\columnwidth}
%	\includegraphics[width=\columnwidth]{figures/TPRF-Spaces-ANCE-Effectiveness_trec_dl_2020.pdf}
% 	\caption{TREC DL 2020}
%	\label{fig:spaces-trec-2020}
%	\end{subfigure}
%\caption{Model sizes for TPRF-ANCE and ANCE-PRF and associated variations w.r.t to R@1000 and nDCG@10.}
%\label{fig:spaces}
%\end{figure}

Figure~\ref{fig:spaces} studies the variations of TPRF model sizes (which depend on the parameters of the transformer, specifically layers and heads), and reports also the model sizes of ANCE-PRF and associated variants. For TPRF, we consider only models that had a higher effectiveness than the corresponding dense retriever during training as evaluated on validation on XXX.


%Figure~\ref{fig:spaces} reports the model sizes with respect to the different dense retrievers that the TPRF is trained on. For ANCE-PRF and associated variations, we use the model checkpoints provided by the original authors in the respective original papers. For TPRF, we report all the model sizes that we have trained with respect to the different base dense retrievers in a single box.

We first start by comparing the ANCE-PRF~\cite{yu2021improving}, DistilBERT-PRF~\cite{li2021improving}, TCTV2-PRF~\cite{li2021improving}, with our TPRF models on top of each base dense retrievers, thus answering RQ1: how does TPRF compare to other DR PRF models, in terms of model size. Either ANCE-PRF and associated variations, or TPRF models trained a new query encoder to generate new query representations based on the original query and feedback passages, but they use different initial models. ANCE-PRF and associated variations use the query encoder from the base dense retriever as the starting point for subsequent training. On the contrary, TPRF uses a vanilla transformer model without any pre-training. Therefore, model sizes of ANCE-PRF and associated variations are determined by the original query encoder size, whereas the TPRF's model sizes are determined by the layers and attention heads in the model: these settings can be adjusted accordingly to obtain larger models or smaller models.

From Figure~\ref{fig:spaces}, we can clearly see that either TPRF-ANCE or TPRF-TCTV2 are both smaller than the respective ANCE-PRF and TCTV2-PRF models. TPRF-DistilBERT, however, is always larger than the DistilBERT-PRF model. 
%HERE WE WANTED A COMMENT ON DISTILBERT

Note that smaller models do not necessarily achieve worse results than larger models: in fact, even the smallest TPRF model (size of 299.2MB) can outperform the respective base dense retriever over several metrics across both datasets. But the smallest TPRF model is trading effectiveness for space (and lower query latency); therefore, it suffers from marginal loss in effectiveness compared to the respective ANCE-PRF and variations in exchange for a smaller model size.

In summary, in answer to RQ1, we conclude that our TPRF leads to better effectiveness even with smaller model size compared to the base dense retrievers, but it suffers from marginal effectiveness losses in exchange of memory savings compared to the respective ANCE-PRF and variations. This trade-off, however, is especially useful in memory-constrained settings: one can train a smaller TPRF model, thus forgoing some effectiveness, but still can get improvements over the base dense retriever models.

\subsection{Comparison w.r.t. Query Latency}

We now compare the efficiency of TPRF with respect to ANCE-PRF~\cite{yu2021improving}, DistilBERT-PRF~\cite{li2021improving}, and TCTV2-PRF~\cite{li2021improving}, as shown in Figure~\ref{fig:latency}.

Because of the input limit constraint, ANCE-PRF and its variants have a nearly constant inference time when the input limit is reached. For TPRF, the inference time increases with tee increase in number of feedback passages considered. However, the TPRF inference time is substantially lower than either of the ANCE-PRF and variants models even with more PRF feedback passages. For ANCE-PRF, DistilBERT-PRF, and TCTV2-PRF, the query latency is determined by the length of the input and the inference speed of the original dense retriever query encoders: when input length increases, the inference time also drastically increases. For example, with 3 feedback passages, the ANCE-PRF's inference time increases by nearly 40x compared to the ANCE model with only the query to encode. Our TPRF model's input length is not affected by how many feedback passages are used: more feedback passages only increase thhe number of the rows in the input matrix. According to our results, even with 100 feedback passages, the inference time of TPRF is still substantially lower than ANCE-PRF with only 10 feedback passages. Since  TPRF is based on a vanilla transformer model, the inference speed is remains the same regardless of te dense retriever used. We conducted extensive analysis of the efficiency for TPRF and other dense retriever PRF models in Section~\ref{sec:dis}.

\subsection{Comparison w.r.t. Model Effectiveness}

%\begin{figure*}
%	\begin{subfigure}
%	\centering
%	\includegraphics[width=\textwidth]{figures/effectiveness_trec_dl_2019.pdf}
% 	\caption{TREC DL 2019}
%	\label{fig:text-prf-depths-trec-2019}
%	\end{subfigure}
%	\begin{subfigure}
%	\centering
%	\includegraphics[width=\textwidth]{figures/effectiveness_trec_dl_2020.pdf}
% 	\caption{TREC DL 2020}
%	\label{fig:text-prf-depths-trec-2020}
%	\end{subfigure}
%	\caption{Variance in effective of TPRF models based on training with different parameter settings. Each boxplot represents the distribution of the maximum result per evaluation metric across all the training parameters.}
%	\label{fig:effectiveness}
%\end{figure*}


Figure~\ref{fig:effectiveness} shows the variance in effectiveness of TPRF over TREC DL 2019 and 2020. We observer that our TPRF are stable across the best checkpoints for each training setting (the interquartile range) over all evaluation metrics, with few exceptions such as TREC 2019 over RR and Recall@100. We also observe that TPRF tend to outperform dense retrievers (the solid lines) in terms of recall and nDCG, and perform on par or even better than dense retrievers with PRF in terms of nDCG and RR. Lastly, TPRF consistently outperforms BM25+RM3 across all metrics and datasets, with the exception of recall where BM25+RM3 is better than TPRF-ANCE.

\begin{table*}
	\centering
	\footnotesize
	\caption{Effectiveness of dense PRF methods, bold values are the best for that metric and dataset. Statistical significant differences ($p<0.05$) are indicated using the superscript character corresponding to each method. \todo{HANG: run stat sign.}}
	\resizebox{!}{0.065\textwidth}{%
		\input{tables/results_best.tex}
	}
	\label{tbl:effectiveness}
\end{table*}

Following previous research~\cite{yu2021improving}, Table~\ref{tbl:effectiveness} shows the checkpoints with the best results achieved by TPRF in terms of nDCG@10. We observe that TPRF-DistilBERT and TPRF-TCTV2 are consistently on par with or outperform DistilBERT-PRF and TCTV2-HN+-PRF in terms of nDCG metrics. On the other hand, TPRF-ANCE tend to be worse than ANCE-PRF, with the exception of R@1000 in TREC DL 2019 where TPRF-ANCE substantially outperforms ANCE-PRF.


==> tables/results_median.tex <==
\begin{tabular}{llrrrrrrr}
\toprule
{} &               Model\_Display &      MAP &       RR &   R@1000 &   nDCG@1 &   nDCG@3 &  nDCG@10 &  nDCG@100 \\
\midrule
0  &                        ANCE &  0.36110 &  0.92010 &  0.66100 &  0.72090 &  0.67650 &  0.64520 &   0.55400 \\
1  &                    ANCE-PRF &  0.40700 &  0.91750 &  0.71370 &  0.73260 &  0.68780 &  0.68070 &   0.59500 \\
2  &                        BM25 &  0.37730 &  0.82450 &  0.73890 &  0.54260 &  0.52300 &  0.50580 &   0.50180 \\
3  &                    BM25+RM3 &  0.42700 &  0.81670 &  0.78820 &  0.54650 &  0.51950 &  0.51800 &   0.52860 \\
4  &     H12\_L12\_ANCE3\_R\_10\_EP50 &  0.38745 &  0.85690 &  0.69110 &  0.63950 &  0.64000 &  0.64060 &   0.55645 \\
5  &       H4\_L6\_ANCE3\_R\_10\_EP50 &  0.37360 &  0.91955 &  0.66780 &  0.68220 &  0.65565 &  0.64270 &   0.55390 \\
6  &      H6\_L10\_ANCE3\_R\_10\_EP10 &  0.36825 &  0.85995 &  0.68350 &  0.60080 &  0.62700 &  0.62745 &   0.54080 \\
7  &      H6\_L10\_ANCE3\_R\_10\_EP50 &  0.38360 &  0.87780 &  0.68740 &  0.63950 &  0.63920 &  0.63160 &   0.55600 \\
8  &  H6\_L8\_ANCE10\_R\_10\_EH2\_EP50 &  0.38155 &  0.76865 &  0.78410 &  0.65120 &  0.65705 &  0.64185 &   0.56265 \\
9  &   H6\_L8\_ANCE1\_R\_12\_EH2\_EP50 &  0.37995 &  0.82150 &  0.77315 &  0.70540 &  0.66755 &  0.65120 &   0.56575 \\
10 &   H6\_L8\_ANCE3\_R\_10\_EH2\_EP50 &  0.38525 &  0.77025 &  0.77155 &  0.64340 &  0.64715 &  0.64500 &   0.56400 \\
11 &       H6\_L8\_ANCE3\_R\_10\_EP10 &  0.37150 &  0.86820 &  0.66745 &  0.62790 &  0.64320 &  0.62795 &   0.54655 \\
12 &       H6\_L8\_ANCE3\_R\_10\_EP50 &  0.38900 &  0.87930 &  0.68625 &  0.62790 &  0.64805 &  0.64090 &   0.55910 \\
13 &   H6\_L8\_ANCE5\_R\_10\_EH2\_EP50 &  0.38555 &  0.76040 &  0.78060 &  0.63760 &  0.64435 &  0.64435 &   0.56915 \\
0  &                        ANCE &  0.40760 &  0.79070 &  0.77640 &  0.73460 &  0.70820 &  0.64580 &   0.56790 \\
1  &                    ANCE-PRF &  0.44520 &  0.83710 &  0.81480 &  0.80250 &  0.74500 &  0.69480 &   0.59470 \\
2  &                        BM25 &  0.28560 &  0.65850 &  0.78630 &  0.57720 &  0.50210 &  0.47960 &   0.49020 \\
3  &                    BM25+RM3 &  0.30190 &  0.63600 &  0.82170 &  0.56480 &  0.47400 &  0.48210 &   0.50770 \\
4  &     H12\_L12\_ANCE3\_R\_10\_EP50 &  0.39525 &  0.72740 &  0.77530 &  0.66205 &  0.65825 &  0.62000 &   0.55095 \\
5  &       H4\_L6\_ANCE3\_R\_10\_EP50 &  0.39935 &  0.80525 &  0.77985 &  0.75465 &  0.69450 &  0.63425 &   0.54795 \\
6  &      H6\_L10\_ANCE3\_R\_10\_EP50 &  0.39720 &  0.72920 &  0.77760 &  0.67280 &  0.67080 &  0.62340 &   0.55450 \\
7  &  H6\_L8\_ANCE10\_R\_10\_EH2\_EP50 &  0.39365 &  0.69165 &  0.78950 &  0.63890 &  0.64615 &  0.61750 &   0.55985 \\
8  &   H6\_L8\_ANCE1\_R\_12\_EH2\_EP50 &  0.40750 &  0.76890 &  0.78715 &  0.71755 &  0.66555 &  0.63275 &   0.56015 \\
9  &   H6\_L8\_ANCE3\_R\_10\_EH2\_EP50 &  0.40670 &  0.74805 &  0.78630 &  0.69290 &  0.66920 &  0.62580 &   0.55880 \\
10 &       H6\_L8\_ANCE3\_R\_10\_EP50 &  0.40570 &  0.73810 &  0.78740 &  0.67435 &  0.67400 &  0.63015 &   0.56435 \\
11 &   H6\_L8\_ANCE5\_R\_10\_EH2\_EP50 &  0.40125 &  0.72870 &  0.78615 &  0.66050 &  0.66425 &  0.61730 &   0.55885 \\
2  &         DistilBERT-Balanced &  0.47610 &  0.95100 &  0.78260 &  0.75580 &  0.74940 &  0.72100 &   0.63600 \\
3  &              DistilBERT-PRF &  0.48740 &  0.86240 &  0.85650 &  0.76360 &  0.77170 &  0.73580 &   0.65400 \\
4  &       H12\_L12\_DB3\_R\_10\_EP50 &  0.45615 &  0.94850 &  0.76245 &  0.74030 &  0.73610 &  0.72020 &   0.62485 \\
5  &         H4\_L6\_DB3\_R\_10\_EP50 &  0.42990 &  0.94555 &  0.74795 &  0.75970 &  0.72040 &  0.68410 &   0.60385 \\
6  &        H6\_L10\_DB3\_R\_10\_EP50 &  0.46070 &  0.93750 &  0.77290 &  0.75580 &  0.75350 &  0.71680 &   0.62920 \\
7  &    H6\_L8\_DB10\_R\_12\_EH2\_EP50 &  0.46070 &  0.79225 &  0.83500 &  0.68990 &  0.71155 &  0.70485 &   0.63480 \\
8  &     H6\_L8\_DB1\_R\_10\_EH2\_EP50 &  0.45130 &  0.88735 &  0.83220 &  0.77130 &  0.72175 &  0.70285 &   0.63130 \\
9  &     H6\_L8\_DB3\_R\_10\_EH2\_EP50 &  0.46420 &  0.85035 &  0.84010 &  0.75970 &  0.75715 &  0.71890 &   0.63625 \\
10 &         H6\_L8\_DB3\_R\_10\_EP50 &  0.46095 &  0.94595 &  0.76670 &  0.74420 &  0.74215 &  0.70805 &   0.62540 \\
11 &     H6\_L8\_DB5\_R\_10\_EH2\_EP50 &  0.45545 &  0.82590 &  0.82845 &  0.73640 &  0.73260 &  0.70380 &   0.63030 \\
2  &         DistilBERT-Balanced &  0.46980 &  0.83500 &  0.87270 &  0.75930 &  0.74260 &  0.68540 &   0.63460 \\
3  &              DistilBERT-PRF &  0.48360 &  0.85250 &  0.86580 &  0.77470 &  0.74590 &  0.69770 &   0.63080 \\
4  &       H12\_L12\_DB3\_R\_10\_EP50 &  0.44645 &  0.82635 &  0.83655 &  0.72530 &  0.72850 &  0.67375 &   0.59335 \\
5  &         H4\_L6\_DB3\_R\_10\_EP50 &  0.43240 &  0.83135 &  0.84235 &  0.77470 &  0.72645 &  0.65470 &   0.58255 \\
6  &        H6\_L10\_DB3\_R\_10\_EP50 &  0.45655 &  0.84285 &  0.85365 &  0.76695 &  0.75175 &  0.68215 &   0.60705 \\
7  &    H6\_L8\_DB10\_R\_12\_EH2\_EP50 &  0.46710 &  0.82935 &  0.85250 &  0.74690 &  0.75115 &  0.69230 &   0.61095 \\
8  &     H6\_L8\_DB1\_R\_10\_EH2\_EP50 &  0.44685 &  0.83805 &  0.84465 &  0.75620 &  0.72230 &  0.66140 &   0.60270 \\
9  &     H6\_L8\_DB3\_R\_10\_EH2\_EP50 &  0.43795 &  0.83845 &  0.83955 &  0.77470 &  0.73635 &  0.66930 &   0.59950 \\
10 &         H6\_L8\_DB3\_R\_10\_EP50 &  0.46505 &  0.84695 &  0.86570 &  0.77160 &  0.73470 &  0.68865 &   0.62000 \\
11 &     H6\_L8\_DB5\_R\_10\_EH2\_EP50 &  0.45595 &  0.81295 &  0.84740 &  0.74690 &  0.73430 &  0.67975 &   0.61010 \\
2  &      H12\_L12\_TCT3\_R\_10\_EP50 &  0.44155 &  0.94020 &  0.74810 &  0.76360 &  0.72685 &  0.70780 &   0.62600 \\
3  &        H4\_L6\_TCT3\_R\_10\_EP50 &  0.43170 &  0.94380 &  0.73525 &  0.75580 &  0.74435 &  0.70220 &   0.62330 \\
4  &       H6\_L10\_TCT3\_R\_10\_EP50 &  0.45450 &  0.94570 &  0.75790 &  0.76360 &  0.75075 &  0.73275 &   0.63620 \\
5  &   H6\_L8\_TCT10\_R\_12\_EH2\_EP50 &  0.47060 &  0.87040 &  0.83850 &  0.77130 &  0.75485 &  0.72545 &   0.64850 \\
6  &    H6\_L8\_TCT1\_R\_10\_EH2\_EP50 &  0.45730 &  0.87420 &  0.82090 &  0.77910 &  0.74640 &  0.71750 &   0.63055 \\
7  &    H6\_L8\_TCT3\_R\_10\_EH2\_EP50 &  0.45190 &  0.84790 &  0.82865 &  0.75580 &  0.73750 &  0.71550 &   0.63165 \\
8  &        H6\_L8\_TCT3\_R\_10\_EP50 &  0.46980 &  0.95810 &  0.76805 &  0.77520 &  0.73975 &  0.71560 &   0.64330 \\
9  &    H6\_L8\_TCT5\_R\_10\_EH2\_EP50 &  0.45645 &  0.84380 &  0.82935 &  0.74030 &  0.72160 &  0.70870 &   0.63735 \\
10 &                   TCTV2-HN+ &  0.46250 &  0.97670 &  0.76020 &  0.80230 &  0.74100 &  0.72040 &   0.63180 \\
11 &               TCTV2-HN+-PRF &  0.47840 &  0.87250 &  0.85190 &  0.75970 &  0.76100 &  0.74110 &   0.65840 \\
2  &      H12\_L12\_TCT3\_R\_10\_EP50 &  0.44245 &  0.85310 &  0.80645 &  0.80865 &  0.74960 &  0.67505 &   0.58565 \\
3  &        H4\_L6\_TCT3\_R\_10\_EP50 &  0.43490 &  0.81170 &  0.81225 &  0.75620 &  0.71645 &  0.65795 &   0.57680 \\
4  &       H6\_L10\_TCT3\_R\_10\_EP50 &  0.44930 &  0.83355 &  0.81320 &  0.78090 &  0.73190 &  0.67315 &   0.58880 \\
5  &   H6\_L8\_TCT10\_R\_12\_EH2\_EP50 &  0.46325 &  0.85505 &  0.82435 &  0.80095 &  0.75145 &  0.68670 &   0.60285 \\
6  &    H6\_L8\_TCT1\_R\_10\_EH2\_EP50 &  0.47120 &  0.85795 &  0.83380 &  0.79320 &  0.73175 &  0.67655 &   0.60470 \\
7  &    H6\_L8\_TCT3\_R\_10\_EH2\_EP50 &  0.45680 &  0.86210 &  0.81425 &  0.79940 &  0.74830 &  0.68240 &   0.58930 \\
8  &        H6\_L8\_TCT3\_R\_10\_EP50 &  0.46790 &  0.83935 &  0.83440 &  0.77780 &  0.73770 &  0.68760 &   0.61005 \\
9  &    H6\_L8\_TCT5\_R\_10\_EH2\_EP50 &  0.46070 &  0.84040 &  0.82440 &  0.78700 &  0.74205 &  0.68230 &   0.59580 \\
10 &                   TCTV2-HN+ &  0.47540 &  0.83920 &  0.84290 &  0.79320 &  0.71990 &  0.68820 &   0.62060 \\
11 &               TCTV2-HN+-PRF &  0.49320 &  0.85090 &  0.84000 &  0.80250 &  0.77450 &  0.71150 &   0.62910 \\
\bottomrule
\end{tabular}

